Deep Orthogonal Decompositions for Convective Nowcasting

Near-term prediction of the structured spatio-temporal processes driving our climate is of profound importance to the safety and well-being of millions, but the prounced nonlinear convection of these processes make a complete mechanistic description even of the short-term dynamics challenging. However, convective transport provides not only a principled physical description of the problem, but is also indicative of the transport in time of informative features which has lead to the recent successful development of ``physics free'' approaches to the now-casting problem. In this work we demonstrate that their remains an important role to be played by physically informed models, which can successfully leverage deep learning (DL) to project the process onto a lower dimensional space on which a minimal dynamical description holds. Our approach synthesises the feature extraction capabilities of DL with physically motivated dynamics to outperform existing model free approaches, as well as state of the art hybrid approaches, on complex real world datasets including sea surface temperature and precipitation.

==> lit_review/lit_review.tex <==
\section{Lit Review}

\begin{itemize}
    \item \textbf{Bezenac et al.} \cite{de2018deep} \\
    This approach uses a convolution-deconvolution (transposed conv.) CNN to attempt to capture spacial variation by claiming to incorporate physics into the loss function. They place a discretised \textit{warping scheme} by linear advection-diffusion into the loss function via a regularisation term on the motion field. \\ \\
    \textsc{Background Summary} \\ \textit{Advection} in transports some conserved quantity, $I$, via \textit{bulk motion}, i.e. for small variations $\Delta x$, $\Delta t$ conservation is expressed as $I(x,t) = I(x+\Delta x, t+\Delta t)$ which after applying a first order approximation of the RHS and reordered we obtain the \textit{advection equation} (or \textit{Brightness Constancy Constraint Equation}), $$\frac{\delta I}{\delta t}+(w \cdot \nabla) I = 0$$ with $\nabla$ denoting the gradient operator, $w$ our motion vector we can use to forecast $I$. \\
    
    \textit{Diffusion} corresponds to the \textit{spreading out} of conserved $I$, i.e. from high to low areas of concentration. Incorporating with transport results: $$\frac{\delta I}{\delta t} + (w. \nabla) I = D \nabla^2 I$$ with $\nabla^2$ the Laplacian operator and $D$ diffusion coefficient (with $D\to0$ transport eq. is clearly recovered). \\
    % \james{we're restricting flow of the transport by fixing it to account for a scaled ($D$) second derivative (Laplacian) of the conserved quantity} \\
    
    \textsc{Novelty} \\
    They claim for any initial condition $I_0 \in L^1 (\mathbb{R}^2)$ with $\lim_{x\to\pm \infty}=0$, $\exists I(x,t)$ a unique global soln to the advection-diffusion eq where $$I(x,t) = \int_{\mathbb{R}^2} k(x-w, y)I_0(y)dy$$ with $k(u,v)$ either an RBF kernel or $\mathcal{N}(x-w, 2Dt)$. This forms their motivation for a warping scheme, discretising the above and using their outputs from the CNN as initial conditions. \\
    
    \textsc{Highlighted Reviewer Comments} \hfill \href{https://openreview.net/forum?id=By4HsfWAZ}{\texttt{openreview.net}}
    \begin{displayquote}
    Most classical variational assimilation schemes are stochastic in nature, notably by incorporating uncertainties in the observation or physical evolution models. It is still unclear how those uncertainties can be integrated in the model \\
    {\color{red}This is the next step of our work. We could introduce uncertainties in different forms. We started to work on a variant of this model using a scheme similar to conditional VAE (Variational Auto Encoder) with the idea that the model should be able to predict multiple potential vector flow candidates instead of a mean value. VAEs allow sampling from noise distributions and then generating diverse candidates.} \\
    
    In the regularization scheme - equation 6 - you are using the gradient and the divergence. With respect to what quantity (e.g. the input?) are you taking the gradient, and if it is the input, what is exactly is the divergence than when the input is not the cartesian coordinates but numerical values? \\
    {\color{red}Gradient and divergence are computed wrt to the spatial variables x and y. To be more precise :
 $$\left \| \nabla w \right \|^2 = (\frac{\partial u }{\partial x})^2 + (\frac{\partial u }{\partial y})^2 + (\frac{\partial v }{\partial x})^2 + (\frac{\partial v }{\partial y})^2$$}

    \end{displayquote}
    
    \item \textbf{Wang et al.} \cite{wang2020towards} \\
    This work claims to produce a NN for approximating turbulent flow. Physics are attributed to two areas of their novelty:
    \begin{enumerate}
        \item their \texttt{Conv TF-Net} loss includes a governing equation (continuity, $\nabla \cdot \boldsymbol{w} = 0$),
        \item their network architecture is justified with the \textit{Hybrid RANS-LES Coupling} method.
    \end{enumerate}
    .\\
    
    \textsc{Background Summary} \\
    Let $\boldsymbol{w}$ be the vector velocity field for flow with two components $(u, v)$, i.e. velocity along $(x, y)$ respectively. Then the governing equations for the Releigh-Benard convection (RBC) model of turbulent convection are as follows:
    \begin{align*}
        &\nabla \cdot \boldsymbol{w} = 0 && \text{Continuity} \\
        &\frac{\partial \boldsymbol{w}}{\partial t}+(\boldsymbol{w} \cdot \nabla) \boldsymbol{w}=-\frac{1}{\rho_{0}} \nabla p+\nu \nabla^{2} \boldsymbol{w}+f && \text{Momentum} \\
        &\frac{\partial T}{\partial t}+(\boldsymbol{w} \cdot \nabla) T=\kappa \nabla^{2} && \text{Temperature}
    \end{align*}
    These are effectively ignored for the rest of the paper and they claim they model RBC with a Boussinesq approximation (which then results in a divergence-free flow $\nabla \cdot \boldsymbol{w} = 0$ everywhere).
    
    Justification for a three-level merged U-net is sourced from a description of \textit{Reynolds-averaged Navier–Stokes} (RANS) and \textit{Large Eddy Simulation} (LES). These two methods are brought together in a \textit{hybrid coupling}. RANS decomposes turbulent flow into a time-averaged mean flow $\bar \boldsymbol{w}$ and fluctuating quantity $\boldsymbol{w}'$ failing to account for broadband unsteadiness and intermittency. LES uses scaled spatial filtering expressed as a convolution product normally taken as Guassian.  LES is more accurate but also computationally more expensive. The Hybrid coupling takes first a LES (spatial pass) over $\boldsymbol{w}$ to form an intermediate $\boldsymbol{w*}$ then apply RANS (temporal averaging pass). This is claimed as less expensive and than pure LES. \\
    
    \textsc{Novelty} \\
    Their novelity is claimed as realisation of the spatial filtering process as one convolutional layer with a single 5×5 filter to each input image. Then another convolutional layer for temporal filtering with a single 1×1 filter applied to every T images. "The motivation for this design is to explicitly guide the DL model to learn the non-linear dynamics of both large and small eddies as relevant to the task of spatio-temporal prediction". These then share the same decoder and they proform one-step ahead prediction. \\
    
    \textsc{Highlighted Reviewer Comments} \hfill \href{https://openreview.net/forum?id=Hkg5lAEtvS}{\texttt{openreview.net}}
    \begin{displayquote}
    ...I am a not totally convinced since (i) the authors said that their goal is to emulate numerical simulations given 'noiseless observations': how can this be used on a real case then? and (ii) the developed (complex) architecture is still not sufficient to constrain the physical problem, as they had to manually include a regularization term (on the divergence) in the loss: what is the purpose of the 'physically-based network' then, and how can this method be extended to other dynamics? \\
    {\color{red}We are only using the general notion of multiscale dynamics to create this template of 3 networks (for slow, medium and fast scales), which is true, generally speaking, for a wide range of physical systems.}
    \\ 
    \daniel{This is the big problem we keep coming back to with this paper, we won't ever need to worry about
    (i) which gets absorbed in the VAE setup, for (ii)
    we will not claim that any specific architecture
    absoloutely constrains the model with a given physics,
    this would require exact specification of the physics 
    this is unreasonable, rather the physics informs a 
    prior -- i.e. the regularizer, and the what follows is a way to build a model that best gives that prior the
    freedom to express itself if supported by the data,
    but does not leave the model beholden to the physics,
    which is what an overly restrictive architecture would
    do} \\
    
    Do you think that your model is able to learn the underlying physics? If so, do we have access to the latent variables, that would be the state of your system (see \cite{abs-1902-11136})? Such as p and T. \\
    {\color{red}Our work implicitly marginalizes out latent variables (p and T). To access those, we would need the initial full state of the system as in I. Ayed paper. We are happy to consider the suggested setup as a future work.} \\
    \daniel{``learning the underlying physics'' is
    something that people get excited about -- personally
    I'm skeptical about the possibility of this, which
    would be *machine learning informed physics* and
    we need to be clear that this isn't what we are doing}
    \end{displayquote}
    
    \item \textbf{Wang et al.} \cite{wang2020incorporating} \\
    Doesn't make the same claims regarding it's capacity to "incorporate physics"
    \textsc{Background Summary} \\ 
    
    \textsc{Novelty} \\
    
\end{itemize}
